ManipTrans: Efficient Dexterous Bimanual Manipulation Transfer via Residual Learning

Human hands play a central role in interacting, motivating increasing research in dexterous robotic manipulation. Data-driven embodied AI algorithms demand precise, large-scale, human-like manipulation sequences, which are challenging to obtain with conventional reinforcement learning or real-world teleoperation. To address this, we introduce ManipTrans, a novel two-stage method for efficiently transferring human bimanual skills to dexterous robotic hands in simulation. ManipTrans first pre-trains a generalist trajectory imitator to mimic hand motion, then fine-tunes a specific residual module under interaction constraints, enabling efficient learning and accurate execution of complex bimanual tasks. Experiments show that ManipTrans surpasses state-of-the-art methods in success rate, fidelity, and efficiency. Leveraging ManipTrans, we transfer multiple hand-object datasets to robotic hands, creating DexManipNet, a large-scale dataset featuring previously unexplored tasks like pen capping and bottle unscrewing. DexManipNet comprises 3.3K episodes of robotic manipulation and is easily extensible, facilitating further policy training for dexterous hands and enabling real-world deployments.

==> sec/XX_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/rebuttal_main.tex <==
We thank the reviewers \textbf{\color[RGB]{34,125,81}xm2b} (\Rone), \textbf{\color[RGB]{0,80,255}XCuM} (\Rtwo), and \textbf{\color[RGB]{233,138,36}6uB9} (\Rthree) for their valuable feedback. They note our idea as ``intuitive" and ``innovative" [\Rone, \Rthree], our method as ``effective" and ``efficient" [\Rone, \Rtwo], our dataset as a ``helpful contribution" [\Rtwo, \Rthree], and our results as ``precise," ``agile," and performing well across embodiments [\Rone]. If this rebuttal increases confidence, we respectfully invite reviewers to \highlight{raise their scores} and \highlight{recommend a strong accept}.

% We will include clarifications below in the revision.

\noindent{\Rtwo, \Rthree:} \textit{\underline{Bimanual tasks with real-world deployment}} are demonstrated in \cref{fig:qualitative}. We conduct experiments with two Realman arms and a pair of \textit{upgraded version} of Inspire Hands (same configuration yet adding tactile sensors), showcasing dexterous manipulation that, to the best of our knowledge, \highlight{has not previously been achieved}. For instance, in ``open the toothpaste", the left hand stably holds the tube while the right hand's thumb and index finger flexibly \textit{pop open} the tiny cap—\highlight{motions difficult to capture via teleoperation}. We will post more videos on website.


\noindent{\Rone:} \textit{\underline{Applying residual policy to retargeted joint angles.}} We apologize for the misunderstanding. The ``Retarget + Residual" results appear in main paper Tab.~{\color{cvprblue}{1}} and Supp. Sec.~{\color{cvprblue}{C.1}}. While ``Retarget + Residual" performs comparably to our method on simpler tasks (\eg, ``rotate a mouse"), \method demonstrates superior performance on more complex tasks, possibly due to our imitator incorporates \highlight{additional dynamic information}, whereas retargeting relies solely on static joint angles. This highlights our method's key novelty over other residual action-based approaches.

\noindent{\Rone:} \textit{\underline{Grasping process.}} We appreciate the opportunity to clarify that our method \highlight{corrects arbitrary, noisy hand-interaction MoCap data into physically plausible motion} without predefined stages such as ``approaching-grasping-manipulation." For ``cap the pen" (main paper Fig.~{\color{cvprblue}{1}} and Supp. video), the left hand smoothly grasps and lifts the cap. \dataset \highlight{focuses more on dexterous manipulation} after grasping (see \cref{fig:qualitative}), as high-quality manipulation data remain scarce compared to grasping data.

\noindent{\Rone:} \textit{\underline{Minor jitter}} arises from the RL policy's direct output. We experimentally find applying a simple first-order low-pass filter ($\alpha=0.5$) effectively reduces jitter with minimal impact on accuracy. We will update videos accordingly.

\noindent{\Rtwo:} \textit{\underline{Floating wrists vs. fixed arms.}} We experimentally find that dual-arm configurations heavily influence success rates because their DoFs, size, and installation setup vary. As an exploratory work, \method seeks \highlight{a more generalizable transfer approach} by relaxing arm constraints rather than limiting itself to a specific robotic arm configuration. Indeed, arms move slower than wrists, so we do not enforce strict temporal alignment for highly dynamic sequences.

% >>>
\noindent{\Rtwo:} \textit{\underline{Explanation of deployment.}} We apologize for the omission. Beyond arm speed limitations, real-world deployment faces IK failures and arm collisions, which we partially mitigate by validating motion sequences in Mujoco first. However, Sim2Real gap persists, such as actuation differences between real robotic hands and simulations (\eg, Inspired Hand's linear servo actuator) and the complexity of friction modeling. We will provide more thorough explanations and failure cases in the final version. We believe bridging these gaps requires industry-academia collaboration, and we hope our work represents a\del{ small but} meaningful step in this direction.

\noindent{\Rtwo:} \textit{\underline{Some training details of the imitator}} appear in Sec.~{\color{cvprblue}{3.2}} (Data Augmentation). We will release full training code.

\noindent{\Rtwo:} \textit{\underline{``Verification of the dataset"}} involves testing \method on only a subset of the dataset to evaluate generalizability (\eg, using articulated objects in ARCTIC). We plan to integrate more hand-object interaction datasets into \dataset and welcome community collaboration.


\noindent{\Rtwo:} \textit{\underline{Learning curve graph}} shows convergence trends. We will add further quantitative analysis in the final version.

\noindent{\Rtwo:} \textit{\underline{Clarifications in experiments.}} We appreciate your insightful suggestion and will reorganize these sections.


\noindent{\Rthree:} \textit{\underline{Contact force feedback}} is not used in real-world deployment, as we currently replay \dataset's trajectory. However, the \textit{upgraded} Inspire Hands incorporate tactile sensors on the skin, \highlight{allowing for the collection of fine-grained contact information} during manipulation.


\noindent{\Rthree:} \textit{\underline{PPO algorithm}} is widely adopted in imitation learning [{\color{cvprblue}20},{\color{cvprblue}21},{\color{cvprblue}42},{\color{cvprblue}43},{\color{cvprblue}84}-{\color{cvprblue}86},{\color{cvprblue}126},{\color{cvprblue}127}], optimizing policy via clipping to preserve TRPO's trust-region principle while reducing overhead and instability. [{\color{cvprblue}18}] provides a thorough benchmark of RL algorithms for dexterous manipulation, quantitatively demonstrating that the PPO series exhibits reduced hyperparameter sensitivity, along with notable stability, sample efficiency, and suitability for high-dimensional control. We appreciate the suggestion to clarify our choice.

\noindent{\Rthree:} \textit{\underline{Designing metrics for morphological differences}} is challenging. We supplement [{\color{cvprblue}68}]'s metrics with $E_{ft}$ to evaluate fingertip positions, as human and robotic hands generally align in fingertip positions during manipulation.

\noindent{\Rthree:} \textit{\underline{Task types in evaluation.}} Sorry for the confusion. We follow the official OakInk v2 train/test split. Bimanual tasks in test set include cutting fruit, uncapping alcohol lamp, \etc.\del{ The complete list will be provided in the final version.}


\begin{figure}[t]
    \centering
    \vspace{0.0002em}
    \includegraphics[width=1.0\linewidth]{figure/rebuttal.pdf}
    \captionsetup[figure]{name={Fig.},labelsep=period}
    \caption{\textbf{Screenshots from real-world bimanual manipulation deployment videos.} The {\color[RGB]{255,123,172}red} box shows the human hands motion, and the {\color[RGB]{251,176,59}orange} box provides a close-up of the dexterous hands.  {\color[RGB]{102,102,102}{\faSearchPlus}}}
    \vspace{-1.2875em}
    \label{fig:qualitative}
\end{figure}



==> table/cmp_dataset.tex <==
\begin{table}[b]
    \rowcolors{4}{WhiteGray}{White}
    \renewcommand{\arraystretch}{1}
    \begin{center}
    \resizebox{1.0\linewidth}{!}
    {
        \setlength{\tabcolsep}{9pt}
        {
        \begin{tabular}{cccccc}
        \toprule
        Dataset & Bimanual & Transfered & \#Task & \#Seq & \#Frame \\
        % \hhline{~~~~--}
        \midrule
         DexMG~\cite{jiang2024dexmimicgen}    &\greencheck      & \greencheck         & 9     &  12k    &5M\\
         \dataset       &\greencheck    &\greencheck        & 36         & 3.3K   & 1.4M \\
         \bottomrule
        \end{tabular}
        }
    }
    \caption{Comparisons with different dexterous manipulation datasets. \ph{2}}
    \label{tab:cmp_dataset}
    \end{center}
\end{table}
